TiDAL: Learning Training Dynamics for Active Learning

Active learning (AL) aims to select the most useful data samples from an unlabeled data pool and annotate them to expand the labeled dataset under a limited budget. Especially, uncertainty-based methods choose the most uncertain samples, which are known to be effective in improving model performance. However, AL literature often overlooks training dynamics (TD), defined as the ever-changing model behavior during optimization via stochastic gradient descent, even though other areas of literature have empirically shown that TD provides important clues for measuring the sample uncertainty. In this paper, we propose a novel AL method, Training Dynamics for Active Learning (TiDAL), which leverages the TD to quantify uncertainties of unlabeled data. Since tracking the TD of all the large-scale unlabeled data is impractical, TiDAL utilizes an additional prediction module that learns the TD of labeled data. To further justify the design of TiDAL, we provide theoretical and empirical evidence to argue the usefulness of leveraging TD for AL. Experimental results show that our TiDAL achieves better or comparable performance on both balanced and imbalanced benchmark datasets compared to state-of-the-art AL methods, which estimate data uncertainty using only static information after model training.

==> Algorithms/1_TiDAL.tex <==
\RestyleAlgo{ruled}
% \begin{wrapfigure}{R}{0.56\textwidth}
% \begin{minipage}[c]{0.56\textwidth}
\begin{algorithm}[H]
\small
\caption{Training Procedure of TiDAL}\label{alg:1_tidal}
\KwIn{labeled training data $\gD$, number of epochs $T$, balancing factor $\lambda$}
\KwOut{target classifier $f$, TD prediction module $m$}
 initialize $f$ and $m$\\
 \For{$t$=$1$,$2$,$\cdots$, $T$}{
    \For{given sample $(x,\vy)\in\sD$}{
        compute predicted probability $\vp^{(t)}(y|x)$ using $f$\\
        compute TD $\widehat{\vp}^{(t)}(y|x)$ $\leftarrow{\sum_{i=1}^{t}\vp^{(i)}(y|x)/t}$\\
        compute predicted TD $\Tilde{\vp}^{(t)}_m(y|x)$ using $m$\\
        compute $L_{\mathrm{target}}\leftarrow{L_{\mathrm{CE}}(\vp^{(t)},\vy)}$\\
        compute $L_{\mathrm{module}}\leftarrow{L_{\mathrm{KL}}(\widehat{\vp}^{(t)}||\Tilde{\vp}^{t}_m)}$\\
        compute $L\leftarrow{L_{\mathrm{target}}+\lambda L_{\mathrm{module}}}$\\
        update $f$ and $m$ using $\min_{f,m}L$\\
    }
 }
\end{algorithm}
% \end{minipage}
% \end{wrapfigure}

==> Figures/x_Pilot_Study_TD.tex <==
\begin{figure*}[t] %%% t: top, b: bottom, h: here
\centering
\begin{subfigure}{.245\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics[width=\textwidth]{Figures/9_3_1_Pilot_Study_Entropy.pdf}}
  \caption{$H^{(t)}$}
  \label{fig:9_3_1}
\end{subfigure}
\begin{subfigure}{.245\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics[width=\textwidth]{Figures/9_3_2_Pilot_Study_Entropy_TD.pdf}}
  \caption{$H_\text{TD}$}
  \label{fig:9_3_2}
\end{subfigure}
\begin{subfigure}{.245\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics[width=\textwidth]{Figures/9_3_3_Pilot_Study_Margin.pdf}
  }
  \caption{$M^{(t)}$}
  \label{fig:9_3_3}
\end{subfigure}%
\begin{subfigure}{.245\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics[width=\textwidth]{Figures/9_3_4_Pilot_Study_Margin_TD.pdf}}
  \caption{$M_\text{TD}$}
  \label{fig:9_3_4}
\end{subfigure}
\caption{
    Class-wise average scores $\mathbb{E}_{x \sim \mathcal{D}_c}[*]$ for each score, where $\mathcal{D}_c$ is the subset of dataset $\mathcal{D}$ with true label $c$.
}
\label{fig:9_3_pilot_study_td}
\end{figure*}

==> Figures/x_Training_Procedure.tex <==
\begin{figure}[t] %%% t: top, b: bottom, h: here
\centering
\includegraphics[width=\columnwidth]{Figures/9_4_Training_Procedure.pdf}
\caption{Training procedure of our proposed TiDAL.
}
\label{fig:9_4_model_architecture}
\end{figure}




% \subfloat[]{\includegraphics[width=0.33\columnwidth]{Figures/5_1_Ablation_CIFAR10.pdf}\label{fig:5_1_ablation_cifar10}}
% \subfloat[]{\includegraphics[width=0.33\columnwidth]{Figures/5_2_Ablation_CIFAR100.pdf}\label{fig:5_2_ablation_cifar100}}
% \subfloat[]{\includegraphics[width=0.33\columnwidth]{Figures/5_3_2_Ablation_kldiv.pdf}\label{fig:5_3_ablation_kldiv}}
% \caption{
%     (a, b) Relative accuracy improvement curves of a single run on different query strategies.
%     $H_m$ and $M_m$ uses the TD prediction module $m$'s outputs for the entropy and the margin, respectively, which is the same to our TiDAL.
%     In contrast, $H_f$ and $M_f$ uses the classifier $f$'s outputs.
%     Total of 4 query strategies are tested on CIFAR10 and CIFAR100.
%     (c) KL divergence $L_\text{KL}$ with the final TD prediction $\Tilde{\mathbf{y}}^{(T)}$ of the TD prediction module $m$.
%     Same with the $\S$~\ref{subsec:3_1_experimental_setup}, we set the total epoch to be $T=200$.
%     CIFAR10 train dataset is used to train the classifier $f$ and the module $m$, where we plot the average $L_\text{KL}$ of the test set.
%     Blue line shows the divergence between $\Tilde{\mathbf{y}}^{(T)}$ and the actual TD $\bar{\mathbf{y}}^{(t)}$ with respect to epoch $t$.
%     Orange line shows the divergence between $\Tilde{\mathbf{y}}^{(T)}$ and the classifier prediction $\widehat{\mathbf{y}}^{(t)}$ with respect to epoch $t$, i.e., output of the model snapshot at epoch $t$.
% }
% \end{figure}


==> Sections/X_Experiments_Details.tex <==
% \input{Tables/dataset_statistics}
% \section{Experiments Details}\label{appendix:b_expeirments_details}
% We provide the detailed implementations in \url{https://anonymous.4open.science/r/TiDAL-D1BE} and the dataset statistics in Table~\ref{tab:dataset_statistics}.

% \noindent
% \textbf{Absolute accuracy.}
% \Cref{figs:9_appendix_accuracy} shows the absolute accuracy for all the baseline methods.
% Our TiDAL has excellent performance, where the margin strategy works great on CIFAR100 and entropy strategy on iNaturalist2018.
% As mentioned in \cref{subsec:4_3_imbalanced_results}, FashionMNIST with the imbalance ratio of $100$ converges quickly with fewer labeled images.
% Hence, it is more informative to compare in earlier stages of training.

% \noindent
% \textbf{Additional baselines.}
% \Cref{figs:10_appendix_vaal} compares our TiDAL with VAAL \cite{sinha2019variational} and TA-VAAL \cite{kim2021task}.
% Except for the case of CIFAR10 with the imbalance ratio of $100$, both TiDAL strategies excel in performance.
% Note that both VAAL and TA-VAAL use a semi-supervised approach to train the selection module and further leverage the unlabeled data for training.

% \noindent
% \textbf{Additional query strategies.}
% We introduced two strategies: entropy $\widehat{H}$ and margin $\widehat{M}$, in \cref{subsec:3_5_uncertainty_estimation}.
% We further demonstrate various uncertainty estimation strategies as follows:
% \begin{align}
%     &\widehat{M}_0(\Tilde{\mathbf{y}}) = p_m(y=\Tilde{y}|x) - \max_{i \neq \Tilde{y}} p_m(y=i|x),\\
%     &\widehat{P}(\Tilde{\mathbf{y}}, \widehat{y}) = p_m(y=\widehat{y}|x),\\
%     &\widehat{P}_0(\Tilde{\mathbf{y}}) = p_m(y=\Tilde{y}|x),
% \end{align}
% where $\Tilde{y} = \text{argmax}_i \ p_m(y=i|x)$ is the class of the maximum module output.

% $\widehat{M}_0$ is the naive variant of the margin $\widehat{M}$ where it does not utilize the predicted label $\widehat{y}$ of the target classifier $f$.
% It calculates the margin between the biggest and the second biggest outputs of the module $m$.
% $\widehat{P}$ uses the module output on the predicted label $\widehat{y}$ from the target classifier $f$ and $\widehat{P}_0$ is the naive variant of $\widehat{P}$ that uses the maximum output of the module $m$.

% \Cref{figs:11_appendix_strategy} shows the average accuracy of $3$ runs for the entropy $\widehat{H}$ and margin $\widehat{M}$, where we show the accuracy of a single run for other strategies.
% We can observe that the naive variant of the margin $\widehat{M}_0$ generally underperforms compared to the margin $\widehat{M}$ except CIFAR100 with the imbalance ratio of $100$.
% There seems to be no clear dominance between $\widehat{P}$ and its naive variant $\widehat{P}_0$.
% However, both $\widehat{P}$ and $\widehat{P}_0$ perform moderately well on both CIFAR100 and FashionMNIST despite its simplicity.
% Future studies may concentrate on broader query strategies based on various training dynamics and its module predictions.

% \include{Figures/9_appendix_accuracy}
% \include{Figures/10_appendix_vaal}
% \include{Figures/11_appendix_strategy}
% \include{Tables/1_dataset_statistics}

